Digital-Analog Quantum Computing and Algorithms

This Thesis delves into the development and implementation of quantum algorithms using the digital-analog quantum computing (DAQC) paradigm. It provides a comparative analysis of the performance of DAQC versus traditional digital approaches, particularly in the presence of noise sources from current noisy intermediate-scale quantum (NISQ) devices. The DAQC paradigm combines the strengths of digital and analog quantum computing, offering greater efficiency and precision for implementing quantum algorithms on real hardware. The Thesis focuses on the comparison of four relevant quantum algorithms using digital and digital-analog approaches, and the results show significant advantages in favor of the latter. Furthermore, the Thesis investigates the cross-resonance effect to achieve efficient and high-precision Hamiltonian simulations. The findings indicate that the digital-analog paradigm is promising for practical quantum computing applications. Its ability to deliver greater efficiency and accuracy in implementing quantum algorithms on real hardware is a significant advantage over traditional digital approaches.

==> snp/fancySection1.tex <==
% \titleformat{\section}[display]
% {\vspace*{150pt}
% \bf\Huge}
% {\hspace{-72pt}{\textcolor{grey}{\thesection}} \hspace{38pt} {\textcolor{white}{#1}}}
% {0pt}
% {}
% []
% \titlespacing*{\section}{108pt}{10pt}{60pt}[20pt]
%
% %Intro
% \titleformat{\section}[display]
% {\vspace*{190pt}
% \bfseries\sffamily \huge}
% {\begin{picture}(0,0)\put(-50,-25){\textcolor{grey}{\thesection}}\end{picture}}
% {0pt}
% {\textcolor{white}{#1}}
% []
% \titlespacing*{\section}{80pt}{10pt}{50pt}[20pt]
%
% %ch 2
% \titleformat{\section}[display]
% {\vspace*{190pt}
% \bfseries\sffamily \huge}
% {\begin{picture}(0,0)\put(-50,-28){\textcolor{grey}{\thesection}}\end{picture}}
% {0pt}
% {\textcolor{white}{#1}}
% []
% \titlespacing*{\section}{80pt}{10pt}{50pt}[20pt]
%
% %ch 3, 4 y 5
% \titleformat{\section}[display]
% {\vspace*{190pt}
% \bfseries\sffamily \LARGE}
% {\begin{picture}(0,0)\put(-50,-35){\textcolor{grey}{\thesection}}\end{picture}}
% {0pt}
% {\textcolor{white}{#1}}
% []
% \titlespacing*{\section}{80pt}{10pt}{40pt}[20pt]

%Conclusions
%Julen conclusions
\titleformat{\section}[display]
{\vspace*{190pt}
\bfseries\sffamily \huge}
{\begin{picture}(0,0)\put(-50,-25){\textcolor{grey}{\thesection}}\end{picture}}
{0pt}
{\textcolor{white}{#1}}
[]
\titlespacing*{\section}{80pt}{10pt}{50pt}[20pt]


==> snp/fancySection3.tex <==
% \titleformat{\section}[display]
% {\vspace*{150pt}
% \bf\Huge}
% {\hspace{-72pt}{\textcolor{grey}{\thesection}} \hspace{38pt} {\textcolor{white}{#1}}}
% {0pt}
% {}
% []
% \titlespacing*{\section}{108pt}{10pt}{60pt}[20pt]
%
% %Intro
% \titleformat{\section}[display]
% {\vspace*{190pt}
% \bfseries\sffamily \huge}
% {\begin{picture}(0,0)\put(-50,-25){\textcolor{grey}{\thesection}}\end{picture}}
% {0pt}
% {\textcolor{white}{#1}}
% []
% \titlespacing*{\section}{80pt}{10pt}{50pt}[20pt]
%
% %ch 2
% \titleformat{\section}[display]
% {\vspace*{190pt}
% \bfseries\sffamily \huge}
% {\begin{picture}(0,0)\put(-50,-28){\textcolor{grey}{\thesection}}\end{picture}}
% {0pt}
% {\textcolor{white}{#1}}
% []
% \titlespacing*{\section}{80pt}{10pt}{50pt}[20pt]
%
% %ch 3, 4 y 5
\titleformat{\section}[display]
{\vspace*{150pt}
\bfseries\sffamily \LARGE}
{\begin{picture}(0,0)\put(-50,-44){\textcolor{grey}{\thesection}}\end{picture}}
{-25pt}
{\textcolor{white}{#1}}
[]
\titlespacing*{\section}{80pt}{10pt}{40pt}[20pt]
%\titlespacing*{\section}{80pt}{10pt}{40pt}[20pt]

% %Conclusions
% %Julen conclusions
% \titleformat{\section}[display]
% {\vspace*{190pt}
% \bfseries\sffamily \huge}
% {\begin{picture}(0,0)\put(-50,-25){\textcolor{grey}{\thesection}}\end{picture}}
% {0pt}
% {\textcolor{white}{#1}}
% []
% \titlespacing*{\section}{80pt}{10pt}{50pt}[20pt]


==> snp/fancySectionChapter4.tex <==
\titleformat{\section}[display]
{\vspace*{190pt}
\bfseries\sffamily \LARGE}
{\begin{picture}(0,0)\put(-50,-20){\textcolor{grey}{\thesection}}\end{picture}}
{0pt}
{\textcolor{white}{#1}}
[]
\titlespacing*{\section}{80pt}{10pt}{40pt}[10pt]
\vfill

